Fighting Fake News in Encrypted Messaging with the Fuzzy Anonymous Complaint Tally System (FACTS)

Recent years have seen a strong uptick in both the prevalence and real-world consequences of false information spread through online platforms. At the same time, encrypted messaging systems such as WhatsApp, Signal, and Telegram, are rapidly gaining popularity as users seek increased privacy in their digital lives. The challenge we address is how to combat the viral spread of misinformation without compromising privacy. Our FACTS system tracks user complaints on messages obliviously, only revealing the message's contents and originator once sufficiently many complaints have been lodged. Our system is private, meaning it does not reveal anything about the senders or contents of messages which have received few or no complaints; secure, meaning there is no way for a malicious user to evade the system or gain an outsized impact over the complaint system; and scalable, as we demonstrate excellent practical efficiency for up to millions of complaints per day. Our main technical contribution is a new collaborative counting Bloom filter, a simple construction with difficult probabilistic analysis, which may have independent interest as a privacy-preserving randomized count sketch data structure. Compared to prior work on message flagging and tracing in end-to-end encrypted messaging, our novel contribution is the addition of a high threshold of multiple complaints that are needed before a message is audited or flagged. We present and carefully analyze the probabilistic performance of our data structure, provide a precise security definition and proof, and then measure the accuracy and scalability of our scheme via experimentation.

==> checkPoly.tex <==
% !TEX root = ideas.tex
%\newcommand{\anote}[1]{\todo[inline, size=\small, author=Arkady]{#1}}
\newcommand{\tuple}[2]{\langle #1, #2 \rangle }
\newcommand{\tup}[1]{\langle #1, #1 \rangle}
\subsection{Server-Checked Complaints}
\paragraph{A fatal flaw?}
In the process of writing this section, I realized that my approach has a fatal flaw.  The problem is with reusing the same check poly, $cp$, for all messages.  Now, when a party $u_i$ receives any two messages, he can compute two ciphertexts with the same value of $cp(i)$.  He can then subtract these homomorphically, to get a ciphertext with a 0 in the $cp$ slot.  This enables him to change the $p(i)$ value in any subsequent complaint without violating correctness of the check poly.  

\paragraph{Original Scheme:}
One problem that we have is clients submitting invalid complaints.  Ideally, we would like to allow the Server to check whether a complaint is valid without learning what message the complaint corresponds to.

Below is a proposed solution for this, though many details in particular, the originating procedure needs to be optimized.

\paragraph{Crypto Tools:}
We use a secret-key homomorphic encryption (HE) scheme that operates on tuples of values $(x_1,x_2)$.  The HE scheme needs to be able to compute additive homomorphism and one level of multiplications.
We need the following security properties (satisfied by many HE schemes)
\begin{itemize}
\item It is hard for someone not knowing $sk$ to produce a valid ciphertext from scratch
\item When given Enc(f(x)) produced by homomorphism, it is not possible to tell what $f$ was.  A stronger form of this, known as circuit privacy, requires that one (even with $sk$) cannot tell the difference between a freshly encrypted $ct$ and one produced via homomorphism.
\end{itemize}
\paragraph{Setup:}
\begin{enumerate}
\item $S$ generates $sk$ for HE.
\item $S$ picks a random degree $t$ check poly, $cp(x)$.  Let $cp_0,\ldots,cp_t$ be the coefficients of $cp$.
\item When a user $u_i$ joins, $S$ computes $Enc_{sk}(\tup{i} ,Enc_{sk}(\tup{i^2}),\ldots,Enc_{sk}(\tup{i^t})$ and gives these to $u_i$.
\end{enumerate}

\paragraph{Originating a message: $S$ and $u_j$ where $j$ is the originator's ID}
\begin{enumerate}
\item $S$ picks a random degree $t$ poly $p_S(x)$ s.t. $p_S(0)=j$
\item $u_j$ picks a random degree $t$ poly $p_O(x)$ s.t. $p_O(0)=0$
\item $S$ and $u_j$ run a maliciously secure 2-PC where.  I am fairly confident that a generic 2-PC is not needed here, but haven't come up with something better. 
\begin{itemize}
\item $S$ inputs $sk$, $\seckeyserv$, $p_S$, $cp$
\item $u_j$ inputs $p_O$
\item The computation checks that $p_O$ is indeed a poly of degree $t$ with $p_O(0)=0$.  Then, computes $p(x)=p_S(x)+p_O(x)$ by adding the coefficients and then returns to $u_j$ encrypted coefficients of $p(x)$ together with a signature by the server authenticating them.\\
Output (to $u_j$):  \\$c = (Enc_{sk}(\tuple{p_0}{cp_0}), \ldots, Enc_{sk}(\tuple{p_t}{cp_t})), \sigma=Sig_{\seckeyserv}(c)$ 
\end{itemize}
\item $u_j$ includes $(c,\sigma)$ with every copy of the message he sends out.
\end{enumerate}

\paragraph{Complaint:}
To complain about a received message $m$, a party $u_i$ does the following:
\begin{enumerate}
\item $u_i$ first checks that $(c,\sigma)$ included in the message is a valid signature.  If not, he sends the invalid message to $S$.  \anote{May need to include the message in $\sigma$ to prevent replay attack?}
\item $u_i$ uses $Enc_{sk}(\tup{i} ,Enc_{sk}(\tup{i^2}),\ldots,Enc_{sk}(\tup{i^t})$ received from $S$ and $Enc_{sk}(\tuple{p_0}{cp_0}), \ldots, Enc_{sk}(\tuple{p_t}{cp_t})$ received in the message to compute $Enc_{sk}(\tuple{p(i)}{cp(i)})$.
\item $u_i$ sends $Enc_{sk}(\tuple{p(0)}{cp(0)})$ to $S$ who decrypts it and checks that $cp(i)$ is correct.  (Recall that $S$ knows $cp$).
\item If this check passes, $u_i$ does the PIR and write to new location trick to write this complaint to a random location (Note that $S$ will see if he write something other than what he checked in the prior step).  
\end{enumerate}


==> implementation_stats.tex <==

% \subsection{Computational Overhead}

% \begin{figure}
%   \includegraphics[width=\linewidth]{imgs/message_creation.png}
%   \label{fig:message_creation}
% \end{figure}
% In Figure 1 we see the time to run the first part of FACTS, that being $\send(u_1, u_2,m,tag_m)$. Looking at message construction we see that until the actual message content exceeds 64MB, creating and sending a message with the encrypted hash and identity takes sub 100ms, excluding the round trip network communication between the client and server. We see then that when a user wishes to forward a message, they will still call $\send(u_1, u_2,m,tag_m)$, but provide the server arbitrary data, and so if this data is less than 2MB, FACTS will add an overhead of only 5ms to this portion of the messaging system.

% \begin{figure}
%   \includegraphics[width=\linewidth]{imgs/message_check.png}
%   \label{fig:message_check}
% \end{figure}
% Whenever a user receives a message, they must also check the construction of the message to ensure the encrypted identity and signature is valid, and has not been tampered with. We see in Figure 2 that for sub 64MB sized messages, FACTS adds only an overhead of at most 150ms.
% \begin{figure}
%   \includegraphics[width=\linewidth]{imgs/var_filter_size.png}
%   \label{fig:var_filter_size}
% \end{figure}

% \begin{figure}
%   \includegraphics[width=\linewidth]{imgs/var_index_size.png}
%   \label{fig:var_index_size}
% \end{figure}
% Finally, we see in Figure 3 that  when a user wishes to actually report a message, there is almost no overhead, as with a fixed size of 1000 user bits, even when the Bloom filter reaches millions of slots, the process of reporting takes under a microsecond. In Figure 4 when we fix the size of the filter at 1 billion slots, we see even when a user's subset of bits is as large as 5000, the reporting process still takes under 15ms.

% \subsection{Network Overhead}
% 


